Local Type Inference for Context-Free Session Types

We address the problem of local type inference for a language based on System F with context-free session types. We present an algorithm that leverages the bidirectional type checking approach to propagate type information, enabling first class polymorphism while addressing the intricacies brought about by the sequential composition operator and type equivalence. The algorithm improves the language's usability by eliminating the need for type annotations at type application sites.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Farzaneh Derakhshan \& Jan Hoffmann (Eds.): 16th International\\ Workshop on
Programming Language Approaches to Concurrency\\
and Communication-cEntric Software 2025 (PLACES 2025)\\
EPTCS 420, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.420.1}{10.4204/EPTCS.420.1}}

